Does mitigating ML's impact disparity require treatment disparity?

Following related work in law and policy, two notions of disparity have come to shape the study of fairness in algorithmic decision-making. Algorithms exhibit treatment disparity if they formally treat members of protected subgroups differently; algorithms exhibit impact disparity when outcomes differ across subgroups, even if the correlation arises unintentionally. Naturally, we can achieve impact parity through purposeful treatment disparity. In one thread of technical work, papers aim to reconcile the two forms of parity proposing disparate learning processes (DLPs). Here, the learning algorithm can see group membership during training but produce a classifier that is group-blind at test time. In this paper, we show theoretically that: (i) When other features correlate to group membership, DLPs will (indirectly) implement treatment disparity, undermining the policy desiderata they are designed to address; (ii) When group membership is partly revealed by other features, DLPs induce within-class discrimination; and (iii) In general, DLPs provide a suboptimal trade-off between accuracy and impact parity. Based on our technical analysis, we argue that transparent treatment disparity is preferable to occluded methods for achieving impact parity. Experimental results on several real-world datasets highlight the practical consequences of applying DLPs vs. per-group thresholds.

==> preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Standard packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{url}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{bbm}
\usepackage{graphicx}
\usepackage[colorinlistoftodos]{todonotes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Math
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{cor}[theorem]{Corollary}
\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}

% Math operators:
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Comments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newcommand{\alex}[1]{\textcolor{violet}{[Alex: #1]}}
% \newcommand{\julian}[1]{\textcolor{blue}{[Julian: #1]}}
% \newcommand{\zack}[1]{\textcolor{magenta}{[Zack: #1]}}

% % To comment out Sandra todo (or anyone)
% \newcommand{\sandra}[1]{}
% To display Sandra todo
% \newcommand{\sandra}[1]{\textcolor{orange}{[Sandra: #1]}}

% To comment out everyone
\newcommand{\alex}[1]{}
\newcommand{\julian}[1]{}
\newcommand{\zack}[1]{}
\newcommand{\sandra}[1]{}


\usepackage{csquotes}
\newcommand{\yhat}{\hat{y}}
\newcommand{\phat}{\hat{p}}
\newcommand{\vct}{\mathbf }



==> sections/background.tex <==

Automated decision-making systems,
based on ML models, 
are now trusted to make decisions of legal consequence, such as extending lines of credit, 
matching employees with employers, etc.
These systems are typically built atop supervised ML models.
In practice, the ML models 
do not take any actions themselves:
they simply estimate the conditional probability 
of a label given some features.
As a concrete example,
a label might be a binary indicator $\left \lbrace 0, 1 \right\rbrace$ 
of whether a loan defaults, 
and the features might be attributes 
related to a loan applicant's financial history.
Decisions are typically made by feeding the conditional probabilities into some decision rule. 

In the simplest systems, the decision rule consists of a threshold applied to the prediction.
For example, if $\hat P(\textit{default}|\mathbf{x}) > .2 \Rightarrow \textit{reject loan}$.
In many cases, while model outputs are generated programatically,
decisions are made by humans. 
For example recidivism scores 
-- predicted probabilities that an individual
will be rearrested after being released --
are taken into account as one among many criteria 
by judges when making decisions about bail, parole and sentencing.

A major concern is that a decision-making system based on an ML model
might exhibit behavior 
that is unlawful with respect to protected characteristics.
If the model explicitly incorporates a protected characteristic as input,
this amounts to disparate treatment \cite{CivilRights1964, barocas2016big, zafar2017fairness}.
An automated ML-based system can also exhibit disparate impact,
which could arise via several possible mechanisms: 
(i) The choice of the target may be arbitrarily chosen 
among several that are all loose surrogates 
for the real quantity of interest (e.g.~credit-worthiness).
Any one particular choice might then benefit or disadvantage a given group;
(ii) The targets themselves might reflect patterns of historical prejudice.
For example, if members of the dominant group 
are more likely to keep their jobs during a layoff, 
then they may be more likely to repay their loans;
(iii) If a group is grossly under-represented in the dataset, 
that could potentially lead to a model 
that is not as accurate when evaluating members of that group.
In some of the literature on fairness in algorithmic decision-making, 
use of the protected characteristic is called \emph{direct discrimination},
while points (i-iii) are sometime described as \emph{indirect discrimination} \cite{pedreshi2008discrimination,kamishima2011fairness}.


Note that the behavior of an ML model 
depends on the dataset used for training, 
and thus these mechanisms could induce disparate impact absent a data scientist's knowledge. 
As Barocas and Selbst note, 
``honest  attempts  to  certify the absence of prejudice on the
part of those involved in the data
mining process may wrongly confer the 
imprimatur of impartiality on the resulting decisions'' \cite{barocas2016big}.
These issues have come to light starting with the ground-breaking paper \cite{friedman1996bias},
which recognized the ability of computer systems to disparately affect protected groups.
Work specifically focused on discrimination owing to data-mining
became more common following \cite{pedreshi2008discrimination}. 
Recently, several prominent cases of disparate impact 
garnered widespread media attention.
For example, a report on ProPublica 
suggested that automated recidivism risk scores, 
used in sentencing and bail decisions, 
show racial bias \cite{MachineBias20}.
Following the organization of workshops 
and conferences addressing related topics,
research into algorithmic methods for mitigating
disparate impact has accelerated.


==> sections/related.tex <==
% %
% % Alex: I think a good use of this section is to discuss work that
% % isn't already mentioned more naturally elsewhere in the paper.  So stuff like other approaches to fairness and DLPs are already covered by the other sections.  We cite Corbett-Davies a ton.  Kleinberg is cited in connection to notions of fairness and trade-offs between them.  
% %

% \subsection{Disparate Learning Processes}
% calders 


% \subsection{Related Algorithms}
% goh? or is it DLP?  (Alex: I don't think it is)
% bechavod

% \subsection{Other Approaches to Fairness}
% moritz
% or does bechavod go here?
% cynthia

% \alex{With the exception of Cynthia (individual fairness), a survey of other notions already appears in Section 5.3.}

% \subsection{Critical Work}
% nissenbaum
% kleinberg
% corbett

% \begin{itemize}
% \item Friedman Nissenbaum \cite{friedman1996bias}
% \item \textbf{DLPs}
% \item \cite{pedreshi2008discrimination}
% \item \cite{kamiran2009classifying}
% \item \cite{calders2010three}
% \item \cite{luong2011k} %not disp impact
% \item \cite{dwork2012fairness} % individual fairness
% \item \cite{zemel2013learning}
% \item \cite{zafar2017fairness}
% \item \textbf{MITIGATING DISPARATE IMPACT BY USING PROTECTED FEATURE}
% \item \cite{hardt2016equality} % not disparate impact
% \item \cite{dwork2017decoupled} describes decoupling % already cited
% \item \textbf{BACKGROUND ON DISCRIMINATION}
% \item \cite{barocas2016big} % already cited
% \item \cite{USConst} % already cited
% \item \cite{grimmelmann2017incomprehensible} (Zootopia paper) % already cited
% \item \textbf{ANALYSIS}
% \item \cite{kleinberg2016inherent} % already cited
% \item \cite{corbett2017algorithmic} % already cited
% \end{itemize}


% In this section we provide a brief overview 
% of some of the other approaches 
% that have been put forth for trading off 
% between classification performance and impact disparity.  
% One common approach consists of preprocessing 
% or ``massaging'' the training data 
% to reduce the dependence between 
% the resulting model predictions 
% and the sensitive attribute \citep{kamiran2009classifying,kamiran2012data,
% feldman2015certifying,adler2016auditing,
% johndrow2017algorithm}. 
% These methods differ both in terms of 
% what variables are affected by the data processing, 
% and the degree of independence that is achieved.  
% For instance, \citet{kamiran2009classifying} 
% propose flipping the negative labels 
% of some observations in the disadvantaged class.
% \citet{zemel2013learning} proposes 
% learning representations---in this case, cluster assignments---of each example
% such that each example maps to a cluster with some probability, seeking parity in the proportion of each group assigned to each cluster.
% \citet{feldman2015certifying} also investigates 
% transformations of the features $X$ 
% into a new set of features that are 
% constructed to be marginally independent from $Z$.  
% \citet{johndrow2017algorithm} demonstrate 
% how to construct transformations 
% to ensure that the derived features 
% are jointly independent of $Z$, 
% and show that this produces distributional parity 
% of the resulting fitted model. 

% A second common approach 
% is to modify existing classification methods 
% either through post-hoc corrections 
% or in the training stage 
% to constrain the level of impact parity 
% in the resulting model. 
% \citet{kamishima2011fairness, goh2016satisfying, calders2010three,kamiran2010discrimination} 
% consider modifications to methods such as SVM, 
% logistic regression, Naive Bayes, and decision trees.  
% \citet{agarwal2017reductions} 
% show how impact parity constraints 
% can be framed as a cost-sensitive classification problem. 

